Sequential Density Ratio Estimation for Simultaneous Optimization of Speed and Accuracy

Classifying sequential data as early and as accurately as possible is a challenging yet critical problem, especially when a sampling cost is high. One algorithm that achieves this goal is the sequential probability ratio test (SPRT), which is known as Bayes-optimal: it can keep the expected number of data samples as small as possible, given the desired error upper-bound. However, the original SPRT makes two critical assumptions that limit its application in real-world scenarios: (i) samples are independently and identically distributed, and (ii) the likelihood of the data being derived from each class can be calculated precisely. Here, we propose the SPRT-TANDEM, a deep neural network-based SPRT algorithm that overcomes the above two obstacles. The SPRT-TANDEM sequentially estimates the log-likelihood ratio of two alternative hypotheses by leveraging a novel Loss function for Log-Likelihood Ratio estimation (LLLR) while allowing correlations up to $N (\in \mathbb{N})$ preceding samples. In tests on one original and two public video databases, Nosaic MNIST, UCF101, and SiW, the SPRT-TANDEM achieves statistically significantly better classification accuracy than other baseline classifiers, with a smaller number of data samples. The code and Nosaic MNIST are publicly available at https://github.com/TaikiMiyagawa/SPRT-TANDEM.

==> Broader_impact.tex <==
% \section{Broader impact}

% \paragraph{Feedback to the field of neuroscience.}Kira et al \citep{Kirasan}. experimentally showed that the SPRT could explain neural activities in the area LIP at the macaque parietal lobe. They randomly presented a sequence of visual objects with associated reward probability. A natural question arises from here: what if the presented sequence is not random, but a time-dependent visual sequence? Will the neural activity be explained by our SPRT-TANDEM, or will the neurons utilize a completely different algorithm? Our research provides one driving hypothesis to lead the neuroscience community to a deeper understanding of the brain's decision-making system.

% \paragraph{Usage of statistical tests.}As of writing this manuscript, not all of the computer science papers use statistical tests to evaluate their experiments. However, in order to provide an objective comparison across proposed and existing models, running multiple validation trials with random seeds followed by a statistical test is helpful. Thus, the authors hope that our paper stimulates the field of computer science to utilize statistical tests more actively.

% \paragraph{Ethical concern.}The proposed method, SPRT-TANDEM, is a general algorithm applicable to a broad range of serial data, such as auditory signals or video frames. Thus, any ethical concerns entirely depend on the application and training database, not on our algorithm \textit{per se}. For example, if SPRT-TANDEM is applied to a face spoofing detection, using faces of people of one particular racial or ethnic group as training data may lead to a bias toward or against people of other groups. However, this bias is a concern in machine learning in general, not specific to the SPRT-TANDEM.

% \paragraph{Is the SPRT-TANDEM optimal?}The SPRT algorithm is Bayes optimal, or at least asymptotically optimal, even on non-i.i.d. data series as long as LLR is precisely calculated. It indicates that if other methods outperform the SPRT-TANDEM, the LLR estimation might be improved even more. However, because our database has finite video frames, we impose a forced decision if the SPRT-TANDEM used up all the frames (i.e., truncated SPRT. Also see Appendix \ref{app:discussion}), deviating from the SPRT that samples as much as possible to reach one of the two thresholds. The deviation from the original SPRT means that even if the LLR estimation is as precise as possible, the performance might be deteriorated. Thus, at this point, it remains an open question if the SPRT-TANDEM is optimal or not because of multiple factors affecting its performance. In either case, however, the authors are looking forward to a novel method superior to the SPRT-TANDEM in order to stimulate research into sequential density estimation.



==> SPRT_limitations.tex <==
\section{SPRT and its limitations}
The sequential test is a method of statistical inference whose characteristic feature is that the number of observations required by the procedure is not determined in advance of the experiment. SPRT's decision value is the LLR, which tells us under which of the two alternative hypotheses, $H_0$ and $H_1$, the current samples are likely to be generated:
\begin{equation}\label{eq:LLR}
LLR = \frac{
	p(x^{(1)}, ..., x^{(t)}| H_{1})
		}{
	p(x^{(1)}, ..., x^{(t)}| H_{0})
		} \, .
\end{equation}
An advantage of the sequential test, when it is used to test statistical hypotheses, is that tests can be constructed to achieve a user-defined classification accuracy with, on average, a substantially smaller number of observations than in equally reliable test procedures based on a predetermined number of observations. In his textbook \citep{WaldBook}, Abraham Wald compared SPRT to the Neyman-Pearson test, a fixed-sample-size test also based on the LLR. By assigning two decision thresholds for the two hypotheses, $H_{0}$ and $H_{1}$, SPRT achieves the desired classification accuracy with a smaller required sample size compared to that of the Neyman-Pearson test (for the proof, see\citep{Tartakovsky}). Moreover, SPRT has been proven to be Bayes-optimal: among all the existing sequential tests, it gives the greatest lower bound of the expected sample size to achieve the desired classification accuracy \citep{WaldBook,Tartakovsky}.\\
\indent Upon acquisition of each sample data, the LLR, based on which the probability ratio test (PRT) is conducted, is updated. The PRT chooses one of two alternatives: (i) classify the data series into one of the hypotheses according to predefined thresholds or (ii) continue data sampling. The thresholds for $H_0$ and $H_1$ are defined as $A=\log{\frac{1-\beta}{\alpha}}$ and $B=\log{\frac{\beta}{1-\alpha}}$, respectively, where $\alpha$ and $\beta$ are user-defined type1 (i.e., reject $H_0$ when it is true) and type2 (i.e., accept $H_0$ when $H_1$ is true) classification errors. The training dataset is denoted by $\{ (\{x_{i}^{(t)}\}_{t=1}^{T}, Y_i) \}_{i=0}^{N} \in (\mathcal{x}^{T}\times\mathcal{Y})^N$, where $\mathcal{x}$ is the input space, $\mathcal{Y} = \{ H_{0}, H_{\mathrm{1}}\}$ is the label space, and $T, N \in \mathbb{N}$. $T+1$ stands for the number of frames.\\
\begin{figure}[htbp]
\centerline{\includegraphics[width=12cm,keepaspectratio]{../SPRT_concept.png}}
\caption{Conceptual diagram of SPRT. Upon acquisition of each sample, the log likelihood from each hypothesis, $H_1$ or $H_0$, is calculated and updated. Sequential sampling continues until the LLR reaches one of the thresholds, $A$ or $B$. Depending on the time-series data, the time to reach the threshold varies: if the series is easy to classify, it takes only a short time to hit the threshold (early finishing). On the other hand, if the series is difficult to classify, it takes a long time to reach a threshold (late finishing).}
\end{figure}
\indent Although the SPRT has advantages, it has at least two critical problems hampering its practical application. First, SPRT does not provide a way to calculate the LLR. Both Wald's original work and its extensions conduct SPRT with given LLRs. Second, the original SPRT considers i.i.d. data series, which is too crude of an assumption for time series. 

